The generalized orthogonal Procrustes problem in the high noise regime

We consider the problem of estimating a cloud of points from numerous noisy observations of that cloud after unknown rotations, and possibly reflections. This is an instance of the general problem of estimation under group action, originally inspired by applications in 3-D imaging and computer vision. We focus on a regime where the noise level is larger than the magnitude of the signal, so much so that the rotations cannot be estimated reliably. We propose a simple and efficient procedure based on invariant polynomials (effectively: the Gram matrices) to recover the signal, and we assess it against fundamental limits of the problem that we derive. We show our approach adapts to the noise level and is statistically optimal (up to constants) for both the low and high noise regimes. In studying the variance of our estimator, we encounter the question of the sensivity of a type of thin Cholesky factorization, for which we provide an improved bound which may be of independent interest.

==> Abstract.tex <==
We consider the problem of estimating a cloud of points from numerous noisy observations of that cloud after unknown rotations, and possibly reflections.
This is an instance of the general problem of estimation under group action, originally inspired by applications in
%cryo-electron microscopy and
three-dimensional imaging and computer vision.
%Motivated by these applications,
We focus on a regime where the noise level is larger than the magnitude of the signal, so much so that the rotations cannot be estimated reliably.
We propose a simple and efficient procedure based on invariant polynomials (effectively: the Gram matrices) to recover the signal, and we assess it against fundamental limits of the problem that we derive. We show our approach adapts to the noise level and is statistically optimal (up to constants) for both the low and high noise regimes.
In studying the variance of our estimator, we encounter the question of the sensivity of a type of thin Cholesky factorization, for which we provide an improved bound which may be of independent interest.


==> Notations.tex <==
\section{Notations}

\begin{itemize}
\item $\KL$: Kullback-Leibler divergence 
\item $\TV$: Total variation distance
\item $\mathrm{F}$: cumulative distribution function of a standard gaussian
\item  $\norm{.}$: Frobenius norm
\item  $\normop{.}$: operator norm
\item $\dotprod{.,.}$: Euclidean inner product on $d \times k$ real matrices
\item $\mathcal{O}(d)$: orthogonal group of dimension $d$
\item $\mu$: Haar measure on the orthogonal group
\item $G(k,r)$: Grassmannian manifold (all $r$-dimensional linear subspace of $\mathbb{R}^{k}$)
\item $\text{Skew}(d)$: skew symmetric matrices of dimension $d$
\end{itemize}



==> StabCholesky.tex <==
\section{Estimation Algorithm}

\subsection{The Gram Matrix determines the orbits}

Our estimator estimates the Gram matrix of the point clouds.
In this section, we show that estimating the second moment is indeed sufficient to estimate the orbits of 
the point clouds.

\begin{proposition}\label{prop::orbitscharateristics}
Let $X_{1}$ and $X_{2} \in \mathbb{R}^{d \times k}$,
then $X_{1}^{T}X_{1} = X_{2}^{T}X_{2}$ if and only if $\exists Q \in \mathcal{O}(d)$ s.t. $X_{1} = QX_{2}$.
\end{proposition}

In order to prove the statement, we start by reminding the following lemma and its proof.

\begin{lemma}\label{lem::choldecomposition}
Let $A$ be positive semi-definite, of rank $d$.\\
\begin{itemize}
\item (a) There exists at least one upper triangular matrix $R$ with nonnegative diagonal elements such that $A = R^{T}R$
\item (b) There exists a permutation $\Pi$ such that $\Pi^{T}A\Pi$ has a unique Cholesky decomposition, which takes the form:
$$
\Pi^{T}A\Pi = R^{T}R,
$$
with
$$R = \begin{pmatrix}
R_{11} & R_{12} \\
0 & 0
\end{pmatrix},$$

where $R_{1,1}$ is a $d \times d$ upper triangular matrix with positive diagonal elements.

\end{itemize}
\end{lemma}

\begin{proof}
The first statement is easy to prove. The second statement if proven by an explicit construction.
\begin{itemize}
\item (a) Let the symmetric positive semi-definite square root $X$ of $A$ have the $QR$ decomposition $X = QR$
with $r_{ii} \geq 0$. Then $A = X^{2} = X^{T}X = R^{T}Q^{T}QR = R^{T}R$.
\item (b) The result can be found in~\citep{Highan90AnalysisCholesky}.
\end{itemize}
\end{proof}

We then prove proposition \ref{prop::orbitscharateristics}.

\begin{proof}
Let's call $G = X_{1}^{T}X_{1} = X_{2}^{T}X_{2}$.
By lemma \ref{lem::choldecomposition}, it is possible to reorganize the points such that we can write:
$$
G = R^{T}R,
$$
with 

$$R = \begin{pmatrix}
R_{11} & R_{12} \\
0 & 0
\end{pmatrix},$$

where $R_{11}$ is upper triangular of size $d \times d$ with a strictly positive diagonal.
Now let's take $L$ of size $d \times k$ such that $L^{T}L = G$.
$\exists$ a $Q\tilde{R}$ decomposition of $L$ with $Q \in \mathcal{O}(d)$ and $\tilde{R} \in \mathbb{R}^{d \times k}$
with a diagonal strictly positive on the $d \times d$ part.
Now, if we add lines of $0$ at the bottom of $R$, we have a matrix of the shape above, which is unique.
Hence $[R_{1,1} R_{1,2}] = \tilde{R} = Q^{T}L$.
This shows that it is always possible to apply a matrix $Q \in \mathcal{O}(d)$ to $L$ to get an unique cloud.

\end{proof}



\subsection{Estimation Algorithm}

Hence, we reduce the problem of orbit recovery to the problem of estimating the Gram matrix $G$ of each equivalence class.
We build on this observation to propose an algorithm to estimate a representant of each equivalence class.
More precisely, we return an estimator of the unique upper triangular matrix $R$ such that $R^{T}R = G$.

\begin{algorithm}
\caption{Estimation algorithm}\label{alg:estimation}
\begin{algorithmic}[1]
\Procedure{}{}\Comment{} 
\State  \textbf{Compute} $\hat{G} = \dfrac{1}{N}\displaystyle\sum_{i=1}^{N}Y_{i}^{T}Y_{i} - d\sigma^{2}\mathrm{I}_{k}$
\State  \textbf{Compute the Eigenvalue Decomposition of } $\hat{G} = \hat{U}\hat{D}\hat{U}^{T}$
\State \textbf{Keep the $d$ largest nonnegatives eigenvalues of} $\hat{D}$ \textbf{ in matrix } $\hat{D}_{d}$
\State \textbf{Compute the $QR$ decomposition of } $\hat{D}_{d}^{1/2}\hat{U}^{T}$
\State \textbf{Return } $R$
\EndProcedure
\end{algorithmic}
\end{algorithm}

Intuitively, we return an estimator of an invariant of the problem.
In~\citep{Bandeira2018EstimationGroupAction} propose to estimate the moments. 
Our estimator has the advantage of being computationally efficient.
The estimation of an invariant moment if proposed, leveraging the properties of the "median of means" \citep{NemirovskyYudin83OptimizationComplexity}.
The concentration properties of the gaussian distribution for the estimation of a second degree moment 
allow us to consider a simple mean.




\subsection{Stability of the Estimator}

We have a consistent estimator of the Gram matrix. However, we return the Cholesky factor of the Gram matrix, a $k \times k$, rand $d$ matrix.
The following result guarantees that such factorization remains consistent.
The problem of the stability of the Cholesky factorization has been addressed in the positive definite case 
~\citep{Drmacetal94CholeskyPerturbation}, ~\citep{Gilletal96CholeskyPerturbationQuasidefinite}, ~\citep{ChangPaigeStewart96CholeskyPerturbation}.
~\citep{Chang96CholeskyPerturbationBackwardErrors}, ~\citep{ChangStehle10RigorousBoundsMatrixFactorization}.
Surprisingly, to the best of our knowledge this problem has not been investigated in the positive semidefinite case.
Theorem \ref{thm::cholstability} extend the existing results to positive semidefinite matrices.



\begin{theorem}\label{thm::cholstability}
Let $X_{1}$ and $X_{2} \in \mathbb{R}^{d \times k}$, then [STATEMENT NOT EXACT]
\begin{equation}\label{eq::stabChol}
 \norm{X_{1} -  X_{2}} \leq \dfrac{\sigma_{min}(X_{1})}{\sqrt{2}}\left(1 - \sqrt{1 - \dfrac{2\norm{X_{1}^{T}X_{1} - X_{2}^{T}X_{2}}}{\sigma_{min}^{2}(X_{1})}} \right).
\end{equation}
\end{theorem}

The proof of the theorem builds on a proof mechanics giving rigorous, nonasymptotic bouns, proposed by ~\citep{ChangStehle10RigorousBoundsMatrixFactorization} and using the properties of an ad-hoc operator.
We start by stating a useful, preliminary result.

%Definitions:\\
%$\mathrm{H}_{X} = \{ \dot{X} \in \mathbb{R}^{d \times k}: \dotprod{\Omega,X} = 0, \forall \Omega \in \text{Skew}(d)\}$\\
%$\mathcal{N} = \{ G \in \R^{k \times k}: G = G^{T}, G \succeq 0, \text{ rank}(G) = d\}$\\
%$\mathrm{T}_{G}\mathcal{N} = \{\}$\\


\begin{lemma}\label{lem::operatorInverse}
Let $H_{X}$, the set of matrices orthogonal to $\Omega X$, $\forall \Omega \in Skew(d)$
$$\mathrm{H}_{X} = \{ \dot{X} \in \mathbb{R}^{d \times k}: \dotprod{\dot{X},\Omega X} = 0, \forall \Omega \in \text{Skew}(d)\}$$.
Let $\mathcal{N}$ be the manifold of positive semidefinite matrices of rank $d$:
$$\mathcal{N} = \{ G \in \R^{k \times k}: G = G^{T}, G \succeq 0, \text{ rank}(G) = d\}$$
and let  $\mathrm{T}_{G}\mathcal{N}$ be the tangent space at $\mathcal{N}$ in G.
Let $\mathcal{L}_{X}$  be the operator defined by:
$$
\begin{array}[t]{lrcl}
\mathcal{L}_{X} :  & \mathrm{H}_{X} & \longrightarrow & \mathrm{T}_{X^{T}X}\mathcal{N} \\
    &\dot{X} & \longmapsto & X^{T}\dot{X} + \dot{X}^{T}X  
\end{array}
$$
Then $\forall \dot{X} \in \mathrm{Ker}(\mathcal{L}_{X})^{\perp}$
 $$
 \mathcal{L}_{X}(\dot{X} ) \geq \sqrt{2}\sigma_{min}(X)\norm{\dot{X} }
 $$
In other words, the smallest singular value of $\mathcal{L}_{X}$ along the orthogonal of its null space is 
 $$\sqrt{2\lambda_{d}(X^{T}X)} = \sqrt{2}\sigma_{min}(X)$$.
 
\end{lemma}

The above result allows us to the prove theorem \ref{thm::cholstability}.

\begin{proof}
Let $X$ and $Y \in \mathbb{R}^{d \times k}$. Without loss of generality we assume that $XY^{T}$ is symmetric
and that $X$ and $Y$ are rotationally aligned (see the proof of \ref{lem::interm2}).
Let 
$$
Z(t) = (1 - t)X + tY = X + t(Y - X) = X + t\Delta X,
$$

With $\Delta X = Y - X$.
We then have
\begin{align*}
Z(t)^{T}Z(t) &= (X + t\Delta X)^{T}(X + t\Delta X),\\
&= X^{T}X + t(\Delta X^{T}X + X^{T} \Delta X) + t^{2}\Delta X^{T}\Delta X,
\end{align*}

Rearranging we get
$$
Z(t)^{T}Z(t) - X^{T}X - t^{2}\Delta X^{T}\Delta X = t \mathcal{L}_{X}(\Delta X),
$$

Since $\Delta X$ is in the horizontal space at X, is is also orthogonal to the null space of $\mathcal{L}_{X}$.
Where $\mathcal{L}_{X}$ is the operator defined in lemma \ref{lem::operatorInverse}.
Hence
$$
t \Delta X = \mathcal{L}_{X}^{\dagger}\left(Z(t)^{T}Z(t) - X^{T}X - t^{2}\Delta X^{T}\Delta X \right),
$$

which implies
$$
t\norm{\Delta X} \leq \dfrac{1}{\sqrt{2}\sigma_{min}(X)}\left[ \norm{Z(t)^{T}Z(t) - X^{T}X} + t^{2}\norm{\Delta X}\right],
$$
Reorganizing, we get
$$
0 \leq t^{2} \norm{\Delta X}^{2} + \sqrt{2} \sigma_{min}(X) t \norm{\Delta X} + \norm{Z(t)^{T}Z(t) - X^{T}X},
$$

Hence $\forall t \in [0,1]$,  $\norm{\Delta X} \geq 0$ and  is outside the closed interval defined by:
$$\left[\dfrac{\sqrt{2}\sigma_{min}(X) - \sqrt{ 2\sigma_{min}(X)^{2}- 4\norm{Z(t)^{T}Z(t) - X^{T}X}}}{2},\dfrac{\sqrt{2}\sigma_{min}(X) + \sqrt{ 2\sigma_{min}(X)^{2}- 4\norm{Z(t)^{T}Z(t) - X^{T}X}}}{2}\right]$$

$$
t \norm{\Delta X} \leq \dfrac{\sigma_{min}(X)}{\sqrt{2}}\left(1 - \sqrt{1 - \dfrac{2\norm{Z(t)^{T}Z(t) - X^{T}X}}{\sigma_{min}^{2}(X)}} \right)
$$

by taking $t = 1$, we get the final claim:
$$
 \norm{Y -  X} \leq \dfrac{\sigma_{min}(X)}{\sqrt{2}}\left(1 - \sqrt{1 - \dfrac{2\norm{Y^{T}Y - X^{T}X}}{\sigma_{min}^{2}(X)}} \right)
$$

\end{proof}


\subsection{Noise regimes}

\begin{proposition}
We can find two noise regimes:
\begin{itemize}
\item  $\sigma^{2} >> 2\dfrac{\lVert X \rVert_{F}^{2}}{pk}$, in which case the variance of the estimator will be $O(\sigma^{4})$
\item $\sigma^{2} << 2\dfrac{\lVert X \rVert_{F}^{2}}{pk}$, in which case the variance of the estimator will be $O(\sigma^{2})$
\end{itemize}

\end{proposition}

\begin{proof}
The proof relies on the computation of the Mean Square Error of the estimator of the Gram matrix proposed in
\ref{alg:estimation}. The details of this computation can be found in Appendix \ref{appendix::MSE}
\end{proof}




==> Synchronization.tex <==
\section{Impossibility of the estimation of rotations in low SNRs}

%The most natural approach consists in estimating the rotations first, and then aligning the observations using the estimated rotations and average.
% - indeed, that what MLE would do: here's the cost function (it's a non convex problem), and notice that if one knew $Q_{1}, ..., Q_{N}$, then the MLE estimator for X would be ...; 


%One natural way to tackle problem \ref{eq::description} consists in 
%estimating each rotation and the matrix $X$.
%This can be done through the computation of the maximum likelihood estimator:
%\begin{equation}\label{eq::MLE}
%\underset{X \in \R^{d \times k},Q_{1},...,Q_{N} \in \mathcal{O}(d)}{\mathrm{argmin}} \sum_{i=1}^{N}\norm{Y_{i} - Q_{i}X}^{2}.
%\end{equation}
%Problem \ref{eq::MLE} is non-convex. 
%One way to overcome the non-convexity consists in anchoring $Q_{1} = I_{d}$, and
%seeing the $K-1$ rotations and the matrix $X$ as fixed parameters.
%Once the rotations $Q_{2}$,...,$Q_{K}$ are estimated, the matrix $X$ is estimated by:
%$$
%\hat{X} = \dfrac{1}{N} \sum_{i=1}^{N}\hat{Q}_{i}^{T}Y_{i},
%$$
%where $\hat{Q}_{i}$ is the maximum likelihood estimator of $Q_{i}$.
%Equivalently, this consists on solving the following, non convex, optimization problem:
%\begin{equation}\label{eq::Gro1}
%\min_{Q_{1},...,Q_{N} \in \mathcal{O}(d)} \sum_{i \neq j}\norm{Q_{i}Y_{i} - Q_{j}Y_{j}}^{2},
%\end{equation}
%or equivalently:
%\begin{equation}\label{eq::Gro2}
%\max_{Q_{1},...,Q_{N} \in \mathcal{O}(d)} \sum_{i \neq j}\dotprod{Q_{i}Y_{i},Q_{j}Y_{j}}.
%\end{equation}
%This problem was investigated by
%~\TODO{!!citet changed into citep!!} \citep{nemirovski2007quadratic}, showing a deep connection 
%with the behavior of the sum of random matrices. 
%This work was later improved by ~\TODO{!!citet changed into citep!!} \citep{Mansocho2010momentinequalities}.
%Such problem can be cast as a generalization of the little Grothendieck problem~\citep{khot2012grothendieck}, ~\citep{naor2013efficient}.
%A natural way to deal with the non convexity and the exponentially large size of the search space 
%is to study a convex relaxation of \eqref{eq::Gro2}.
%Following the line initiated by the seminal work of ~\TODO{!!citet changed into citep!!} \citep{goemans1995maxcut}, ~\TODO{!!citet changed into citep!!} \citep{bandeira2016Grothendieck} 
%proposed a semidefinite relaxation of  \ref{eq::Gro2}.
%~\citep{singer2011eigen}, ~\citep{WangSingerWen13OrientationCryoEM} 
%has focused on solving the following, non convex, optimization problem
%The most natural way to solve the problem consists in computing the maximum likelihood estimator.
%This implies considering the rotations of each observation as a parameter of the problem, and estimating them.
%One natural method to estimate such parameters, is the alignment approach.
%However, for high noise regimes such approach fails.



==> VarianceWignerApprox.tex <==
How good is this estimator of $\sigma$? We provide a partially heuristic discussion, supported with numerical simulations.
%: we flag the parts that are not completely rigorous explicitly, and we illustrate the accuracy of the predictions we formulate in Section~\ref{sec::noiseRegimes}.
Following computations deferred to Appendix~\ref{appendix::MSE}, whenever $N \gg \sigma^{4} \gg \norm{X}^{2}$
and $\sigma^{4} \gg \sigma^{2}$ we have that,
%\TODO{How come we need $k$ smaller than $\sigma^4$? If $\sigma$ is very small, shouldn't our job be easy for any $k$? In fact, shouldn't a large $k$ always make our life easier? Or is this a typo and should we have $k$ instead of $\sigma^4$ here, as below?}
\begin{equation}\label{approxWigner}
\hat{M}_{N} \approx X^{T}X + \sigma^{2}dI_{k} + H,
\end{equation}
%\TODO{So, the scaling factor here is not adaptive: we need $N \gg \sigma^4$. In Appendix G, do we get an adaptive statement? If so, we could reformulate here to point this out, for example saying that we run the computations here in the low SNR regime, and concluding the section with a word about the other regime.} 
where $H = \sqrt{\frac{\sigma^{4}d}{N}}W$ is a rescaled Wigner matrix $W$, that is, $W = W^T$, its off-diagonal entries are distributed as $W_{i,j} = W_{j,i} \sim \mathcal{N}(0,1)$, 
%\TODO{Here you write $W_{i,j}$ instead of $W_{ij}$: is this consistent throughout the paper?->Yes.}
and its diagonal entries obey $W_{i,i} \sim \mathcal{N}(0,2)$, all independent.
%Here, we would like to stress that such approximation is not valid for $\sigma^2 \gg \sigma^4$.
%\TODO{This last statement is hard to parse, and it's difficult to imagine why. It's saying that the discussion only works for large noise, right? WHat can be said about our estimator of $\sigma$ for the case where $\sigma$ is small? Is it easy then?}
%Hence, for large $N$: 
%\begin{equation}\label{approxWigner} -- SAME LABEL AS ABOVE!
%\Tr{\hat{M}_{N}} \approx \Tr{X^{T}X} + dk\sigma^{2}+ \Tr{H}.
%\end{equation}
 %\TODO{begin reformulation}\\

The eigenvalues of $W$ follow a semicircle law: with high probability, they lie (mostly) within the interval $[-2\sqrt{k}, 2\sqrt{k}]$ (see equation~\eqref{appendix::semiCircle} in Appendix~\ref{appendix::MSE}), in which case the eigenvalues of $H$ are no larger than $2\sigma^2 \sqrt{\frac{dk}{N}}$.
If this is small, by Weyl's inequality,
 the eigenvalue $\lambda_{i}$ is close to the $i$th eigenvalue of $X^{T}X + d\sigma^{2}I_{k}$, which implies that 
 $\sum_{i=1}^{d}\lambda_{i} \approx \mathrm{Tr}(X^{T}X) + d^{2}\sigma^{2}$.
% \TODO{Hence, when $k \gg d$, we can make the assumption that subtracting the $d$ largest eigenvalues is not going
% to affect the trace of the stochastic component $H$, that is,---I do not understand this}
Moreover~\eqref{approxWigner} implies that $\Tr{\hat{M}_N} \approx \Tr{X^{T}X} + \sigma^{2}d^{2}k +  \Tr{H}$.
Hence, we can make the approximation
 $$\Tr{\hat{M}_N} - (\lambda_1 + \cdots + \lambda_d) \approx (dk - d^2)\sigma^{2} + \Tr{H}.$$
 Plugging this expression and the approximation~\eqref{approxWigner} into~\eqref{eq::SigmaEstimator} we get that:
  %\TODO{Missing argument here}\\
%Hence $\lambda_1 + \ldots + \lambda_d \approx \mathrm{Tr}(X^{T}X)$.
  %\TODO{end reformulation}\\
%Plugging this expression and the approximation~\eqref{approxWigner} into~\eqref{eq::SigmaEstimator}, we get that:
\begin{align*}
\hat \sigma_N^2 &\approx \sigma^{2} + \dfrac{1}{d(k - d)}\Tr{H}.
\end{align*}
Since $\Tr{W}$ is a centered Gaussian with variance $2k$, it follows that, approximately, with $N \gg k \gg d$, the estimator $\hat \sigma_N^2$ is unbiased and has variance
%
%Hence the variance of the estimator behaves like the variance of 
%\begin{align*}
%\dfrac{1}{d(k - d)}\Tr{H} = \dfrac{1}{d(k - d)}\sqrt{\dfrac{d\sigma^{4}}{N}}\Tr{W}.
%\end{align*}
%This implies that the variance of $\hat{\sigma}_{N}^{2}$ is approximately
\begin{align*}
\Var{\hat{\sigma}_{N}^{2}} \approx  \dfrac{2k}{d(k-d)^{2}}\dfrac{\sigma^{4}}{N}. 
\end{align*}
We illustrate the accuracy of those predictions in Figure~\ref{fig::BiasSigma}.
\TODO{We discussed Figure 2 and decided to change it, no? Specifically, this figure does not illustrate the accuracy of the prediction, since the prediction is that the variance is so-and-so, but there is no test of that.}
%and~\ref{fig::VarianceSigma}. \TODO{Ref?}
%\TODO{Add the derivation, starting with the main claim.}
\begin{algorithm}[t]
	\caption{Estimation algorithm with $\sigma$ unknown}\label{alg:estimationnosigma}
	\begin{algorithmic}[1]
		\State Execute steps 1 and 2 of Algorithm~\ref{alg:estimation}.
		\State Define $\hat\sigma_N \geq 0$ such that $\hat\sigma_N^2 = \dfrac{1}{d(k-d)}\Big( \Tr{\hat{M}_N} - (\lambda_1 + \cdots + \lambda_d) \Big)$. %\TODO{here you have hats on lambdas but not in Algo 1?}
		\State Define the scaling factors $\alpha_i = \sqrt{\max(0, \lambda_i - d\hat \sigma_N^2)}$ for $i = 1, \ldots, d$.
		\State Execute step 4 of Algorithm~\ref{alg:estimation}.
	\end{algorithmic}
\end{algorithm}

